Adaptive LiDAR Scanning: Harnessing Temporal Cues for Efficient 3D Object Detection via Multi-Modal Fusion

Multi-sensor fusion using LiDAR and RGB cameras significantly enhances 3D object detection task. However, conventional LiDAR sensors perform dense, stateless scans, ignoring the strong temporal continuity in real-world scenes. This leads to substantial sensing redundancy and excessive power consumption, limiting their practicality on resource-constrained platforms. To address this inefficiency, we propose a predictive, history-aware adaptive scanning framework that anticipates informative regions of interest (ROI) based on past observations. Our approach introduces a lightweight predictor network that distills historical spatial and temporal contexts into refined query embeddings. These embeddings guide a differentiable Mask Generator network, which leverages Gumbel-Softmax sampling to produce binary masks identifying critical ROIs for the upcoming frame. Our method significantly reduces unnecessary data acquisition by concentrating dense LiDAR scanning only within these ROIs and sparsely sampling elsewhere. Experiments on nuScenes and Lyft benchmarks demonstrate that our adaptive scanning strategy reduces LiDAR energy consumption by over 65% while maintaining competitive or even superior 3D object detection performance compared to traditional LiDAR-camera fusion methods with dense LiDAR scanning.

==> sec/checklist.tex <==
\newpage
\section{Reproducibility Checklist}
\subsection*{General Paper Structure}
\begin{enumerate}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced  (yes/partial/no/NA): \textbf{Yes}
 \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no): \textbf{Yes}
 \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no): \textbf{Yes}
\end{enumerate}

\subsection*{Theoretical Contributions}
\begin{enumerate}
    \item Does this paper make theoretical contributions? (yes/no): \textbf{No}
\end{enumerate}
\subsection*{Dataset Usage}
\begin{enumerate}
\item Does this paper rely on one or more datasets? (yes/no) \textbf{Yes}

\item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA): \textbf{Yes}
\item All novel datasets introduced in this paper are included in a data appendix (yes/partial/no/NA): \textbf{N/A}
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes (yes/partial/no/NA): \textbf{N/A}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations (yes/no/NA): \textbf{Yes}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available (yes/partial/no/NA). \textbf{Yes}
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing (yes/partial/no/NA): \textbf{N/A}
\end{enumerate}
\subsection*{Computational Experiments}
\begin{enumerate}
\item Does this paper include computational experiments? (yes/no): \textbf{Yes}
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting (yes/partial/no/NA) : \textbf{Yes}
\item Any code required for pre-processing data is included in the appendix (yes/partial/no): \textbf{Yes}
\item All source code required for conducting and analyzing the experiments is included in a code appendix (yes/partial/no): \textbf{Yes}
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes (yes/partial/no): \textbf{Yes}
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no): \textbf{Yes}
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results (yes/partial/no/NA): \textbf{Yes}
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks (yes/partial/no): \textbf{Yes}
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics: \textbf{Yes}
\item This paper states the number of algorithm runs used to compute each reported result (yes/partial/no): \textbf{Yes}
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information (yes/no): \textbf{No}
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank) (yes/partial/no): \textbf{No}
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments (yes/partial/no/NA): \textbf{Yes}
\end{enumerate}
